On Evolving Attention Towards Domain Adaptation

Towards better unsupervised domain adaptation (UDA). Recently, researchers propose various domain-conditioned attention modules and make promising progresses. However, considering that the configuration of attention, i.e., the type and the position of attention module, affects the performance significantly, it is more generalized to optimize the attention configuration automatically to be specialized for arbitrary UDA scenario. For the first time, this paper proposes EvoADA: a novel framework to evolve the attention configuration for a given UDA task without human intervention. In particular, we propose a novel search space containing diverse attention configurations. Then, to evaluate the attention configurations and make search procedure UDA-oriented (transferability + discrimination), we apply a simple and effective evaluation strategy: 1) training the network weights on two domains with off-the-shelf domain adaptation methods; 2) evolving the attention configurations under the guide of the discriminative ability on the target domain. Experiments on various kinds of cross-domain benchmarks, i.e., Office-31, Office-Home, CUB-Paintings, and Duke-Market-1510, reveal that the proposed EvoADA consistently boosts multiple state-of-the-art domain adaptation approaches, and the optimal attention configurations help them achieve better performance.

==> Sections/1_intro.tex <==
\section{Introduction}
%%% \paragraph{the topic and its significance}.
Unsupervised domain adaptation (UDA)~\cite{ganin2015DANN,long2017JAN,long2018CDAN} aims at exploiting the meaningful knowledge from a labelled source domain to facilitate learning on another unlabelled target domain. Generally, researchers focus on learning transferable representations to achieve high accuracy on target domains. A recent research proposes to use attention modules~\cite{wang2019TN,wang2019TADA,li2020DCAN,wang2020DAFD} to further enhance the cross domain feature representation. However, the aforementioned work designs the attention configuration by hand and may falls to a sub-optimal solution in real world application. For example, in Figure~\ref{fig:Motivation}, we observe that on a given UDA task scenario, different configurations of attention module focus on various visual patterns and thus may come out with different accuracies. Therefore, given one arbitrary UDA dataset, a more generalized manner is to automatically find the optimal attention configuration.

%%%%%%%%%%
\input{figures/Motivation}

%%% \paragraph{related work and challenges}
One ideal and widely-used solution is neural architecture search (NAS)~\cite{liu2018DARTS,zoph2018NASNet,real2019EvoNAS,guo2020SPOS}. The goal of NAS is to automatically seek for effective and transferable architectures~\cite{zoph2018NASNet,li2020adapting}.
Nevertheless, existing NAS methods may be ineffective in UDA tasks.
In a conventional NAS setting, we have labelled data on both the training and validation partitions, and assume that the two datasets have little domain shift~\cite{quionero2009dataset}. It means that the architectures optimized on the training domain have little problem to generalize on the validation domain and can be directly evaluated on the validation domain with ground-truth labels. But in an UDA scenario, we have no manual annotation on target domain for training and validation, and there exists relatively larger domain shift between the source and the target domains.
It causes a crucial challenge to evaluate the searched architectures: if we use the labelled data from source domain, the optimized architectures have a risk of overfitting on source domain and being sub-optimal on target domain. Recent NAS literature~\cite{li2020adapting} also points out that existing NAS algorithms are vulnerable to large domain shift.
Besides, we need to design a new search space, which is one important piece of NAS methods, that contains diverse attention configurations for various UDA scenarios.

%%%%%%%%%%
\input{figures/SHOT_vs_SHOTandOurs}

%%% \paragraph{an interesting perspective to study with NAS}
%%% \paragraph{what we done specifically in this paper}
%%% the key idea is to formulate the searching as an optimization problem that seeks to xxx
In this paper, for the first time, we propose a novel and effective NAS algorithm, termed \iMethod, to automatically search configurations of attention module, \ie, the type and position of attention module, for different UDA scenarios.
% The key contributions are a specially designed search space to produce diverse attention configurations and a simple yet effective UDA-oriented evolution-based NAS algorithm.
Specifically, inspired by the progresses of attention modules~\cite{wang2019TADA,li2020DCAN,wang2020DAFD}, we design to search the type and the position of widely-used attention modules~\cite{hu2018SENet,gao2019GSoP}. 
% Intuitively, building on a set of powerful attention modules, we find better configurations of attention module for one given cross-domain scenario with a high probability.
To optimize such attention configuration for UDA tasks, we further propose a new evolution-based NAS method, where we first train the network weights on two domains with arbitrary domain adaptation methods and evaluate the attention configurations by their discrimination on the target domain.
% These criterion are employed to evaluate whether the searched models are optimal on specific UDA tasks.
Experiments on multiple cross-domain benchmarks show that the searched attention configuration via our \iMethod\ benefits several popular domain adaptation methods and lead to better classification performance on target domain.

%%% \paragraph{summary}
The detailed contributions are listed as follows:
\begin{itemize}
    \item We propose a new search space with a set of effective attention modules. The search space covers diverse attention configurations and is able to reinforce representations for UDA tasks.
    
    \item We propose a novel NAS scheme to optimize attention configurations for arbitrary UDA settings. And empirically, we find that the measure of discrimination on target domain is effective to select optimal attention configurations on the target domain.
    
    % \item Together, we present evidence that attention module means a lot in domain adaptation. %, eliminating human experts' effort in designing networks for UDA.
    
    % \item One is for discrimination on target domain. The other is to avoid negative transfer on source domain.
\end{itemize}

Extensive experiments on multiple benchmarks, including Office-Home, Duke-Market1501, and CUB-Paintings, demonstrate that the searched architectures by our NAS algorithm successfully consolidate various popular \SOTA domain adaptation methods~\cite{long2018CDAN,liang2020shot,ge2020MMT,wang2020PAN}) and largely promote their classification performance (see Figure~\ref{fig:SHOT_vs_SHOTandOurs}). We observe that the result gains can be achieved by only introducing a few attention modules in their backbone networks and a moderate increase of FLOPS.
Numerical results also provide practical insights for further research.

==> figures/AccGoesWithPE.tex <==
% \begin{figure*}%[htb]
% % \setlength{\abovecaptionskip}{0pt}
% % \setlength{\belowcaptionskip}{0pt}
%     \centering
%     \subfigure[Pr to Ar]{
%     % \label{analysis:a_distance}
%     \begin{minipage}{0.31\linewidth}
%         \includegraphics[width=1\linewidth]{images/SHOT_PDA_P2A.png}
%         \end{minipage}
%     }
%     \subfigure[Pr to Cl]{
%     % \label{analysis:a_distance}
%     \begin{minipage}{0.31\linewidth}
%         \includegraphics[width=1\linewidth]{images/SHOT_PDA_P2C.png}
%         \end{minipage}
%     }
%     \subfigure[Pr to Rw]{
%         % \label{analysis:lambda}
%         \begin{minipage}{0.31\linewidth}
%         \includegraphics[width=1\linewidth]{images/SHOT_PDA_P2R.png}
%         \end{minipage}
%     }
%     \label{fig:AccGoesWithPE}
%     \caption{Partial-set UDA classification accuracy on target domain goes with the value of performance evaluation $\mathcal{L}_{\Tdomain}^{PE}$. Points indicate the model with different attention configurations and corresponding weights.}
%     \vspace{-3mm}
% \end{figure*}

\begin{figure*}%[htb]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{0pt}
    \centering
    \subfigure[Office-31]{
        \label{fig:Office31_SourceAcc_VS_TargetAcc}
        \begin{minipage}{0.235\linewidth}
        \includegraphics[width=1\linewidth]{images/Office31_SourceAcc_VS_TargetAcc.png}
        \end{minipage}
    }
    \subfigure[Office-31]{
        \label{fig:Office31_Pseudo_TargetAcc}
        \begin{minipage}{0.235\linewidth}
        \includegraphics[width=1\linewidth]{images/Office31_Pseudo_TargetAcc.png}
        \end{minipage}
    }
    \subfigure[Office-Home]{
    \label{fig:OfficeHome_SourceAcc_VS_TargetAcc}
    \begin{minipage}{0.235\linewidth}
        \includegraphics[width=1\linewidth]{images/OfficeHome_SourceAcc_VS_TargetAcc.png}
        \end{minipage}
    }
    \subfigure[Office-Home]{
    \label{fig:OfficeHome_Pseudo_TargetAcc}
    \begin{minipage}{0.235\linewidth}
        \includegraphics[width=1\linewidth]{images/OfficeHome_Pseudo_VS_TargetAcc.png}
        \end{minipage}
    }
    \caption{The rank correlation between the accuracy on target domain and the estimations via $\mathcal{L}_{\Tdomain}^{PE}$. The experiments are conducted in closed-set UDA on Office-31 and Office-Home. Points indicate the model with different attention configurations and their weights.
    }
    \label{fig:AccGoesWithPE}
    \vspace{-2mm}
\end{figure*}

==> figures/ConfusionMatrix_CUBPaintings.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/confusion_matrix_P2C.pdf}
    \caption{The confusion matrix visualization on the fine-grained UDA task of CUB-200-Paintings to CUB-200-2011. \textit{Left}: PAN~\cite{wang2020PAN} on ResNet-50. \textit{Right}: PAN on ResNet-50 with the optimal attention configurations via our method.}
    \label{fig:ConfusionMatrix_CUBPaintings}
    \vspace{-3mm}
\end{figure}

==> figures/SamplingSearchSpace.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/SamplingSearchSpace_TODO.png}
    \caption{A schematic illustration of sampling $\alpha_{i}$, attention type and attention position on one certain backbone network (\eg, ResNet-50) from our proposed search space.}
    \label{fig:SamplingSearchSpace}
    \vspace{-3mm}
\end{figure}

==> figures/TrainingPipeline.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.92\linewidth]{images/TrainingPipeline_TODO.png}
    \caption{A schematic illustration of the proposed UDA-oriented NAS algorithm.
    It consists of four components: 1) \textit{Update seed}: introduce several random seeds and conduct warm-up; 2) \textit{Inference}: evaluate how each seed works in a given UDA task; 3) \textit{Update best}: based on the results of inference, we record the best ones in an output list; 4) \textit{Crossover and mutate}: exploit good seeds and explore poor ones.}
    \label{fig:TrainingPipeline}
    % \vspace{-3mm}
\end{figure*}

==> figures/UDA_and_EvoUDA.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/UDA_and_EvoUDA.png}
    \caption{TODO.}
    \label{fig:UDA_and_EvoUDA}
\end{figure}

==> figures/VisAttention.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{images/VisAttention.pdf}
    \caption{Attention visualization of the last convolutional layer of different networks on the task of Ar$\to$Cl of Office-Home.
    The raw image are three randomly-chosen target images: Bike, Laptop, and Helmet (from top to bottom).
    The rest columns illustrate the attention maps of three different configurations of attention mechanism on ResNet-50, respectively.}
    \label{fig:VisAttention}
    \vspace{-3mm}
\end{figure}

==> figures/tSNE_Office31_AtoW.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/tSNE_Office31_AtoW.png}
    \caption{The t-SNE visualizations of (a) CDAN and (b) CDAN+Ours on the UDA task of \textcolor{blue}{W}$\to$\textcolor{red}{A} from Office-31 dataset. %\textcolor{blue}{Blue} points are source domain data and \textcolor{red}{red} points are target domain data.
    }
    \label{fig:tSNE_Office31_AtoW}
    \vspace{-3mm}
\end{figure}

==> tables/Choices_of_PE.tex <==
\begin{table}
    \centering
    \caption{Comparison of the proposed performance evaluation strategy and two typical ones. The Experiments are conducted on the four closed-set / partial-set UDA settings on Office-Home dataset.}
    \label{tab:Results_choices_of_PE}
    \small{
    \setlength{\tabcolsep}{2.6mm}{
    \begin{tabular}{l|cccc|c}
        \toprule
        A$\to$C & C$\to$P & P$\to$R & R$\to$A & AVG \\
        \hline
        \multicolumn{6}{c}{\textbf{closed-set UDA}} \\
        \hline
        CDAN~\cite{long2018CDAN} & 55.4 & 74.5 & 80.7 & 74.1 & 71.2 \\
        ours & 60.0 & 77.9 & 82.8 & 77.5 & 74.6 \\
        \hline
        \hline
        \multicolumn{6}{c}{\textbf{partial-set UDA}} \\
        \hline
        ETN~\cite{cao2019ETN} & 56.4 & 71.0 & 81.7 & 77.8 & 71.7 \\
        ours & 66.5 & 80.9 & 90.1 & 85.5 & 80.8 \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> tables/Results_CUB200_FGDA.tex <==
\begin{table}
    \centering
    \caption{Accuracy ($\%$) on CUB-Paintings (ResNet-50) and ReID.}
    \label{tab:Results_CUB200}
    \footnotesize{
    \setlength{\tabcolsep}{2.3mm}{
    \begin{tabular}{l|cc|c}
        \toprule
        \multirow{2}{*}{Method} & \scriptsize{CUB-200-2011$\to$} & \scriptsize{CUB-200-Paintings} & \multirow{2}{*}{AVG} \\
         & \scriptsize{CUB-200-Paintings} & \scriptsize{$\to$CUB-200-2011} &  \\
        \hline
        ResNet-50~\cite{he2016resnet} & 47.9 & 36.6 & 42.3 \\
        % x &  &  &  \\
        DANN~\cite{ganin2015DANN} & 57.5 & 43.0 & 50.3 \\
        JAN~\cite{long2017JAN} & 62.4 & 40.4 & 51.4 \\
        MCD~\cite{saito2018MCD} & 63.4 & 43.6 & 53.5 \\
        BSP~\cite{chen2019BSP} & 63.3 & 46.6 & 55.0 \\
        SAFN~\cite{xu2019SAFN} & 61.4 & 48.9 & 55.2 \\
        \hline
        CDAN~\cite{long2018CDAN} & 63.2 & 45.4 & 54.3 \\
        % seed x x x
        % C2P 68.79 67.87 68.30 - 68.32
        % P2C 54.45 53.78 53.31 - 53.84
        +Ours & 68.3 & 53.8 & 61.1 \\
        \hline
        PAN~\cite{wang2020PAN} & 67.4 & 50.9 & 59.2 \\
        % seed 2021, 2020, 2019
        % C2P: 70.20, 69.41, 71.84
        % P2C: 56.35, 55.52, 56.02
        +Ours & \textbf{70.5} & \textbf{56.0} & \textbf{63.3} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-5mm}
\end{table}

==> tables/Results_UDA_for_ReID.tex <==
% \begin{table}
%     \centering
%     \caption{Experimental results ($\%$) of the proposed method and MMT on two popular person re-identification benchmarks.}
%     \label{tab:UDA_for_ReID}
%     \small{
%     \setlength{\tabcolsep}{1.2mm}{
%     \begin{tabular}{l|cccc}
%         \toprule
%         \multirow{2}{*}{Method} & \multicolumn{4}{c}{Market1501 to Duke} \\
%         \cline{2-5}
%          & mAP & top-1 & top-5 & top-10 \\
%         \hline
%         MMT-500-ResNet50 & 63.1 & 76.8 & 88.0 & 92.2 \\
%         MMT-700-ResNet50 & 65.1 & 78.0 & 88.8 & 92.5\\
%         MMT-DBSCAN-ResNet50 &  &  &  & \\
%         MMT-500-IBN-ResNet50 & 65.7 & 79.3 & 89.1 & 92.4 \\
%         MMT-700-IBN-ResNet50 & 68.7 & 81.8 & 91.2 & 93.4 \\
%         MMT-DBSCAN-IBN-ResNet50 &  &  &  & \\
%         \hline
%         MMT-500+Ours & 69.6 & 82.9 & 91.2 & 93.4 \\
%         MMT-700+Ours &  &  &  & \\
%         MMT-DBSCAN+Ours & 71.4 & 82.9 & 91.9 & 94.3 \\
%         \hline
%         \hline
%         \multirow{2}{*}{Method} & \multicolumn{4}{c}{Duke to Market1501} \\
%         \cline{2-5}
%          & mAP & top-1 & top-5 & top-10 \\
%         \hline
%         MMT-500-ResNet50 & 71.2 & 87.7 & 94.9 & 96.9 \\
%         MMT-700-ResNet50 & 69.0 & 86.8 & 94.6 & 96.9 \\
%         MMT-DBSCAN-ResNet50 &  &  &  & \\
%         MMT-500-ResNet50 & 76.5 & 90.9 & 96.4 & 97.9 \\
%         MMT-700-ResNet50 & 74.5 & 91.1 & 96.5 & 98.2 \\
%         MMT-DBSCAN-ResNet50 &  &  &  & \\
%         \hline
%         MMT-500+Ours & 79.9 & 93.4 & 97.7 & 98.5 \\
%         MMT-700+Ours & 78.5 & 93.5 & 97.5 & 98.4 \\
%         MMT-DBSCAN+Ours & 84.3 & 94.2 & 98.2 & 98.8 \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}

\begin{table}
    \centering
    \caption{Results ($\%$) of MMT with different backbones on two person ReID benchmarks. Compared with two typical networks (ResNet-50~\cite{he2016resnet} and IBN-Net-50~\cite{pan2018IBNNet}), the searched networks via our \iMethod\, achieve better results.}
    \label{tab:UDA_for_ReID}
    \footnotesize{
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{ll|cccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Architecture} &  \multicolumn{4}{c}{Market1501 $\to$ Duke} \\
        \cline{3-6}
         &  & mAP & top-1 & top-5 & top-10 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-500}} & ResNet-50 & 63.1 & 76.8 & 88.0 & 92.2 \\
         & IBN-Net-50 & 65.7 & 79.3 & 89.1 & 92.4 \\
         & Ours & 69.6 & 82.9 & 91.2 & 93.4 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-700}} & ResNet-50 & 65.1 & 78.0 & 88.8 & 92.5\\
         & IBN-Net-50 & 68.7 & 81.8 & 91.2 & 93.4 \\
         & Ours & 71.0 & 83.3 & 91.3 & 94.0 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-DBSCAN}} & ResNet-50 & 64.3 & 78.0 & 88.8 & 92.0 \\
         & IBN-Net-50 & 68.8 & 81.4 & 91.1 & 93.9 \\
         & Ours & 71.4 & 82.9 & 91.9 & 94.3 \\
        \hline
        \hline
        \multirow{2}{*}{Method} & \multirow{2}{*}{Architecture} & \multicolumn{4}{c}{Duke $\to$ Market1501} \\
        \cline{3-6}
         &  & mAP & top-1 & top-5 & top-10 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-500}} & ResNet-50 & 71.2 & 87.7 & 94.9 & 96.9 \\
         & IBN-Net-50 & 76.5 & 90.9 & 96.4 & 97.9 \\
         & Ours & 79.9 & 93.4 & 97.7 & 98.5 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-700}} & ResNet-50 & 69.0 & 86.8 & 94.6 & 96.9 \\
         & IBN-Net-50 & 74.5 & 91.1 & 96.5 & 98.2 \\
         & Ours & 78.5 & 93.5 & 97.5 & 98.4 \\
        \hline
        \multirow{3}{*}{\footnotesize{MMT-DBSCAN}} & ResNet50 & 75.6 & 89.1 & 96.2 & 97.6 \\
         & IBN-Net50 & 80.5 & 92.1 & 97.7 & 98.6 \\
         & Ours & 84.3 & 94.2 & 98.2 & 98.8 \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> tables/sup_Results_CUB200_FGDA.tex <==
\begin{table}
    \centering
    \caption{Accuracy ($\%$) on CUB-Paintings (ResNet-50) and ReID.}
    \label{sup_tab:Results_CUB200}
    \small{
    \setlength{\tabcolsep}{2.3mm}{
    \begin{tabular}{l|cc|c}
        \toprule
        \multirow{2}{*}{Method} & \scriptsize{CUB-200-2011$\to$} & \scriptsize{CUB-200-Paintings} & \multirow{2}{*}{AVG} \\
         & \scriptsize{CUB-200-Paintings} & \scriptsize{$\to$CUB-200-2011} &  \\
        \midrule
        % x &  &  &  \\
        CDAN~\cite{long2018CDAN} & 63.2 & 45.4 & 54.3 \\
        % seed x x x
        % C2P 68.79 67.87 68.30 - 68.32
        % P2C 54.45 53.78 53.31 - 53.84
        CDAN+Ours & 68.3 & 53.8 & 61.1 \scriptsize{(+6.8)} \\
        \midrule
        PAN~\cite{wang2020PAN} & 67.4 & 50.9 & 59.2 \\
        % seed 2021, 2020, 2019
        % C2P: 70.20, 69.41, 71.84
        % P2C: 56.35, 55.52, 56.02
        PAN+Ours & 70.5 & 56.0 & 63.3 \scriptsize{(+4.1)} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> tables/sup_Results_Office31.tex <==
\begin{table}
    \centering
    \caption{Accuracy ($\%$) on Office-31 for UDA (ResNet-50).}
    \label{sup_tab:Results_Office31}
    \small{
    \setlength{\tabcolsep}{0.9mm}{
    \begin{tabular}{lccccccc}
        \toprule
        Method & \scriptsize{A$\to$W} & \scriptsize{D$\to$W} & \scriptsize{W$\to$D} & \scriptsize{A$\to$D} & \scriptsize{D$\to$A} & \scriptsize{W$\to$A} & \scriptsize{AVG}\\
        \midrule
        CDAN~\cite{long2018CDAN} & 94.1 & 98.6 & 100.0 & 92.9 & 71.0 & 69.3 & 87.7 \\
        CDAN+Ours & 94.4 & 99.1 & 100.0 & 92.9 & 73.8 & 74.4 & 89.1 \scriptsize{(+1.4)} \\
        \midrule
        SHOT~\cite{liang2020shot} & 90.9 & 98.8 & 99.9 & 93.1 & 74.5 & 74.8 & 88.7 \\
        SHOT+Ours & 94.0 & 97.9 & 100.0 & 94.2 & 74.6 & 74.9 & 89.3 \scriptsize{(+0.6)} \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-4mm}
\end{table}

==> tables/sup_Results_OfficeHome.tex <==
%% result variances??
\begin{table*}
    \centering
    \small{
    \setlength{\tabcolsep}{0.9mm}{
    \caption{Accuracy ($\%$) on Office-Home for UDA, PDA, and ODA methods (ResNet-50).}
    \label{sup_tab:Results_OfficeHome}
    \begin{tabular}{lccccccccccccc}
        \toprule
        \textbf{Closed-set UDA} & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        \midrule
        CDAN~\cite{long2018CDAN} & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8 \\
        CDAN+Ours & 55.4 & 73.4 & 80.4 & 65.8 & 74.5 & 74.9 & 65.1 & 52.4 & 80.7 & 74.1 & 56.6 & 84.2 & 69.8 \scriptsize{(+4.0)} \\
        \midrule
        SHOT~\cite{liang2020shot} & 56.9 & 78.1 & 81.0 & 67.9 & 78.4 & 78.1 & 67.0 & 54.6 & 81.8 & 73.4 & 58.1 & 84.5 & 71.6 \\
        SHOT+Ours & 60.0 & 78.0 & 83.5 & 74.0 & 77.9 & 79.8 & 71.2 & 56.3 & 82.8 & 77.5 & 59.0 & 86.2 & 73.9 \scriptsize{(+2.3)} \\
        % other + Ours &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        % @ 200729, PDA later
        \hline \hline
        Partial-set UDA & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & AVG \\
        \midrule
        ETN~\cite{cao2019ETN} & 59.2 & 77.0 & 79.5 & 62.9 & 65.7 & 75.0 & 68.3 & 55.4 & 84.4 & 75.7 & 57.7 & 84.5 & 70.5 \\
        % SAFN~\cite{xu2019SAFN} & 58.9 & 76.3 & 81.4 & 70.4 & 73.0 & 77.8 & 72.4 & 55.3 & 80.4 & 75.8 & 60.4 & 79.9 & 71.8 \\
        % BA$^{3}$US~\cite{liang2020BA3US} & 60.6 & 83.2 & 88.4 & 71.8 & 72.8 & 83.4 & 75.5 & 61.6 & 86.5 & 79.3 & 62.8 & 86.1 & 76.0 \\
        ETN+Ours & 56.4 & 79.6 & 85.7 & 73.3 & 71.0 & 78.3 & 72.3 & 53.0 & 81.7 & 77.8 & 55.6 & 82.1 & 72.2 \scriptsize{(+1.7)} \\
        \midrule
        SHOT~\cite{liang2020shot} & 62.8 & 84.2 & 92.3 & 75.1 & 76.3 & 86.4 & 78.5 & 62.3 & 89.6 & 80.9 & 63.8 & 87.1 & 78.3 \\
        SHOT+Ours & 66.5 & 84.7 & 89.8 & 80.3 & 80.9 & 86.3 & 83.3 & 64.1 & 90.1 & 85.5 & 61.4 & 89.9 & 80.2 \scriptsize{(+1.9)} \\
        \bottomrule
    \end{tabular}
     % setlength
     % footnotesize
    }
    }
    \vspace{-4mm}
\end{table*}
